The price of debiasing automatic metrics in natural language evaluation

For evaluating generation systems, automatic metrics such as BLEU cost nothing to run but have been shown to correlate poorly with human judgment, leading to systematic bias against certain model improvements. On the other hand, averaging human judgments, the unbiased gold standard, is often too expensive. In this paper, we use control variates to combine automatic metrics with human evaluation to obtain an unbiased estimator with lower cost than human evaluation alone. In practice, however, we obtain only a 7-13% cost reduction on evaluating summarization and open-response question answering systems. We then prove that our estimator is optimal: there is no unbiased estimator with lower cost. Our theory further highlights the two fundamental bottlenecks---the automatic metric and the prompt shown to human evaluators---both of which need to be improved to obtain greater cost savings.

==> arun_theorems.tex <==
\onecolumn

\section{\label{sec:proofs}Proofs}

In this section, we provide proofs for the theorems stated in the main paper.
As many of these proofs are general in nature, we adopt a change of notation to be closer to those used in statistics. 

\subsection{Unbiased estimation.}

Let $x_i \in \sX$ be a set of (ground truth) variables,
let $y_i \eqdef x_i + \s_Y\e_i$ where $e_i$ be some independent zero-mean random variable,
and let $z_i$ be another sequence of random variables with no particular conditions.

A system $S$ comprises of a subset of these indices, $\{x_i: i \in S\} \subseteq \sX$.
Let $\Xb_S = \frac{1}{S} \sum_{i \in S} x_i$ be the average system performance.
Our goal is, given systems $S_1, S_2, \dots$, access to $Y_1, \dots$ and $Z_1, \dots$ is to estimate $\bXb = \Xb_1, \Xb_2, \dots$. \ac{express that $Y_i$ doesn't need to span all samples.}
Furthermore, let the correlation between $X_i$ and $Z_i$ be $\rho_i$.

Let $\delta(\bY, \bZ)$ be an estimator of $\bXb$.
Unbiasedness requires that $\E[\delta(\bY, \bZ)] = \bXb$.
For concreteness, the risk of this estimator is $\E[\|\delta(\bY, \bZ) - \bXb\|^2]$
In this case, a minimum risk estimator using the squared loss is also the minimum variance estimator.

\paragraph{Simple estimator}
Let $\delta(\bY, \bZ) \eqdef (\bYb_1, \dots, \bYb_n)$.
$\delta$ is unbiased.
The variance of $\delta_i$ is:
\[
\Var(\delta_i) = \frac{\s^2_{X_i} + \s^2_Y}{n_i}.
\]

\ac{Technically Stein estimators can be better for $n > 3$ systems\dots}

\paragraph{Simple model-baseline estimator}
Let $\delta(\bY, \bZ) \eqdef (\bZb_1 + \bYb_1 - \bZb_1, \dots)$. \ac{here, the second $\bZb_i$ is restricted to what's been annotated.}

The variance of $\delta_i$ is:
\[
\Var(\delta_i) = \frac{(1-\rho_i^2)\s^2_{X_i} + \s^2_Y}{n_i}.
\]

\paragraph{Optimal model-based estimators}

Let us further assume that both $y_i$ (really $e_i$) and $z_i$ are independent and normally distributed;
  in this scenario, $T = (\bYb, \bZb, S_y, S_z)$ are complete sufficient statistics.
Furthermore, by the magical property of Gaussians, each of these terms is independent of the other.

By Rao-Blackwell, we know that any unbiased function that is only a function of $T$ is optimal.
Let $\delta = \bYb - \bZb'$.

\ac{Stein's shows up here too, but in that case, we consider things that could be unbiased too.}

\section{\label{sec:incomplete}Incomplete}

This section is development space for new material.

\subsection{Incorporating annotator variance}
Broader formulation of annotator variance.

\subsection{Equivariant formulation}
In principle, unbiasedness is too strong a condition for our evaluation metric because it is not important if the metric has been scaled and shifted.
In other words, if $F_i$ is the quality of system $S_i$, then knowing $F'_i \gets \alpha F_i + \beta$ would be just as good, as long as each $F'_i$ respected the same linear transformation.

More formally, let us say that the output $z$ is sampled according to some (unknown) distribution assume $p(z; F)$, then $p(z\given F) = p(\alpha z + \beta \given \alpha F + \beta)$.
$f_i \to \alpha f_i + \beta$ if $F \to \alpha F + \beta$.

A more appropriate formulation then is that of \textit{equivariant estimation}:
(define equivariance).

In this formulation, let $f_i \eqdef f(x_i)$ be the ground truth for $f_i$, and $h_i \eqdef \alpha f_i + \beta + \epsilon$, where $\epsilon$ is some zero mean residual, be human responses.
In other words, the ground truth is \textit{defined} to be some scale/shift of the mean human response: this scaling/shifting is constant across examples.
Without loss of generality, $\alpha = 1$ and $\beta = 0$.

Our question then is, given a series of responses $g_i$, $h_i$ (where $g_i$ comes from the model), what is the minimum risk equivariant (MRE) for $F = \E[f_i]$?
Here, the risk function instead of being squared loss, is $\ell(\frac{\delta - \beta}{\alpha})$ or something like that that is invariant to scaling and shifting in $F$ (as those would result in an appropriate shifting/scaling of $\alpha$ and $\beta$).

\section{Statistical lemmas}

\begin{lemma}[Sufficient statistics for a two-factor Gaussian,unknown mean,  known covariance]%
\label{lem:suff-stats-two-factor}
  Let $y_{uv} = x_u + w_v + r_{uv}$ be a two-factor Gaussian model where $x_u \sim \sN(\mu_X, \sigma_X^2)$, $w_v \sim \sN(0, \sigma_W^2)$ and $r_{uv} \sim \sN(0, \sigma_{R}^2)$ are all drawn independently.
  The covariance of $y_{uv}$ is given by $\Sigma$. 

  Then, the sufficient statistic for the distribution of $\by \given \mu_X$ is $\ones^\top\Sigma^{-1} \by$.
\end{lemma}
\begin{proof}
  We use the Fisher-Neymann factorization theorem:
  \begin{align*}
  \log p(\by \given \mu_X) 
      &= C - \frac{1}{2} (\by - \mu_X \ones)^\top \Sigma^{-1}  (\by - \mu_X \ones) \\
      &= C'(\by) + C''(\mu_X) + (\by^\top \Sigma^{-1} \mu_X \ones) \\
      &= C'(\by) + C''(\mu_X) + \mu_X (\by^\top \Sigma^{-1} \ones) \\
      &= C'(\by) + C''(\mu_X) + \mu_X (T(\by)).
  \end{align*}
  Thus, $T(\by) \eqdef \ones^\top\Sigma^{-1} \by$ is a (complete) sufficient statistic.
  \ac{Show that it is complete.}
\end{proof}

\begin{lemma}[Sufficient statistics for a restricted two-factor Gaussian, unknown mean, unknown covariance]%
\label{lem:suff-stats-two-factor-restricted}

  Similar to \reflem{suff-stats-two-factor},
  let $y_{uv} = x_u + w_v + r_{uv}$ be a two-factor Gaussian model where $x_u \sim \sN(\mu_X, \sigma_X^2)$, $w_v \sim \sN(0, \sigma_W^2)$ and $r_{uv} \sim \sN(0, \sigma_{R}^2)$ are all drawn independently.
  The covariance of $y_{uv}$ is given by $\Sigma$. 
  We assume further structure on $\Sigma$.

  Suppose $y_{uv}$ is the $i$-th response, then
  let $U$ be an indicator matrix where each row $i$ has a single non-zero unit element at the index $u$ and let $V$ be an indicator matrix such row $i$ its a single non-zero unit element at index $v$.
  Further, let we assume that the columns of $U$ are also unique; without loss of generality, $U = I$.
  Responses can still be correlated because they share $w_v$ terms, given by $V$.

  Then, the sufficient statistics for the distribution of $\by \given \mu_X, \Sigma$ are:
  \begin{align*}
    T_1(\by) &= \|\by\|^2 \\
    T_2(\by) &= \|V^\top \by\|^2 \\
    T_3(\by) &= \ones^\top \by \\
    T_4(\by) &= \ones^\top V V^\top \by.
  \end{align*}
\end{lemma}
\begin{proof}
  Note that in this case, the covariance matrix $\Sigma = \sigma^2_X + \sigma^2_R I + \sigma^2_W V V^\top$.

  From \reflem{indicator-matrix}, we have that: 
  \begin{align*}
    \Sigma^{-1} 
      &= ((\sigma^2_X + \sigma^2_R) I + \sigma^2_W V V^\top)^{-1} \\
      &= D^{-1}(I + D' V V^\top)^{-1} \\
      &= D^{-1} I - D^{-1} \frac{D'}{1+D'} V V^\top \\
      &= C I - C' V V^\top,
  \end{align*}
  where it should be noted that $C$ and $C'$ are functions of the unknown parameters $\sigma^2_X$, $\sigma^2_W$ and $\sigma^2_R$.

  Once again, we use the Fisher-Neymann factorization theorem:
  \begin{align*}
  \log p(\by \given \mu_X, \Sigma) 
      &= D(\Sigma) - \frac{1}{2} (\by - \mu_X \ones)^\top \Sigma^{-1}  (\by - \mu_X \ones) \\
      &= D(\Sigma) - \frac{1}{2} (\by - \mu_X \ones)^\top (CI - C' VV^\top) (\by - \mu_X \ones) \\
      &= D'(\mu_X, \Sigma) - \frac{1}{2} (C \|\by\|^2 + 2 C' \|\by V\|^2 - 2 \mu_X \ones^\top \by - 2 \mu_X C' \ones^\top V V^\top \by)\\
      &= D'(\mu_X, \Sigma) - \frac{1}{2} f(T_1(\by), T_2(\by), T_3(\by), T_4(\by)),
  \end{align*}
  where 
    $T_1(\by) = \|\by\|^2$,
    $T_2(\by) = \|V^\top \by\|^2$,
    $T_3(\by) = \|\ones^\top \by\|^2$,
    $T_4(\by) = \|\ones^\top V V^\top \by\|^2$.

  \ac{To show that these are complete.}
\end{proof}

\begin{lemma}[Properties of indicator matrices]%
\label{lem:indicator-matrix}

  An indicator matrix is a matrix such that each row contains exactly one non-zero element which is equal to one.
  Let $U$ be a $m\times n$ indicator matrix where $u(i) \in [n]$ be the index of the unit entry in the $i$-th row.
  Similarly, let $V$ be a $m\times p$ indicator block matrix where $v(i) \in [p]$ is analogously defined.
  Then, the following properties hold:
  \begin{enumerate}
    \item ${(UU^\top)}_{ij} = \I[u(i) = u(j)]$.
    \item ${(U^\top U)} = I$.
    \item $W \eqdef {(U^\top V)}_{ij} = \sum_{k} \I[u(k) = i \band v(k) = j]$.
    \item $W^\top W = \sum{k', k''} \I[u(k') = u(k'')] \I[v(k') = i] \I[v(k'') = j]$.
    \item $W W^\top = \sum{k', k''} \I[v(k') = v(k'')] \I[u(k') = i] \I[u(k'') = j]$.
    \item ${(I + k UU^\top)}^{-1} = I - \frac{k}{k+1} U U^\top$.
  \end{enumerate}
\end{lemma}
\begin{proof}
  The first four results follow from elementary matrix multiplication:
  \begin{align*}
    {(UU^\top)}_{ij}
    &= \sum_{k} U_{ik} U_{jk} \\
    &= \sum_{k} \I[k = u(i)] \I[k = u(j)] \\
    &= \I[u(i) = u(j)] \\
    {(U^\top U)}_{ij}
    &= \sum_{k} U_{ki} U_{kj} \\
    &= \sum_{k} \I[u(k) = i] \I[u(k) = j] \\
    &= \I[i = j] \\
    W 
    &= \sum_{k} U_{ki} V_{kj} \\
    &= \sum_{k} \I[u(k) = i] \I[v(k) = j] \\
    W^\top W
    &= \sum_{k} W_{ki} W_{kj} \\
    &= \sum_{k} \sum_{k'} \I[u(k') = k] \I[v(k') = i] \sum_{k''} \I[u(k'') = k] \I[v(k'') = j] \\
    &= \sum_{k', k''} \I[u(k') = u(k'')] \I[v(k') = i] \I[v(k'') = j] \\
    W W^\top
    &= \sum_{k} W_{ik} W_{jk} \\
    &= \sum_{k} \sum_{k'} \I[u(k') = i] \I[v(k') = k] \sum_{k''} \I[u(k'') = i] \I[v(k'') = k] \\
    &= \sum_{k', k''} \I[v(k') = v(k'')] \I[u(k') = i] \I[u(k'') = j].
  \end{align*}

  The final result follows from the Woodbury matrix identity: 
  \begin{align*}
    {(I + k U U^\top)}^{-1}
    &= I - U {(\frac{1}{k} I +  U^\top U)}^{-1} U^\top \\
    &= I - U {(\frac{1}{k} I + I)}^{-1} U^\top \\
    &= I - \frac{k}{k+1} U U^\top.
  \end{align*}
\end{proof}

\begin{lemma}[Woodbury Matrix Identity]
  Let $A, U, C, V$ be matrix of appropriate dimensions: ${\left(A+UCV\right)}^{-1} = A^{-1} - A^{-1} U {\left(C^{-1}+VA^{-1}U\right)}^{-1} V A^{-1}$. 
\end{lemma}

\begin{lemma}[Non-independence]
  If $U$ and $V$ are indicator matrices then ${(I + k UU^\top + l VV^\top)}^{-1}$ can not be written as linear sequence $\sum_{k,l} f_i(k,l) g_i(U, V)$.
\end{lemma}
\begin{proof}
  Let $k' = \frac{k}{k+1}$.
  \begin{align*}
    {(I + k U U^\top + l VV^\top)}^{-1}
    &= I - k' U U^\top - (I - k' U U^\top) V (\frac{1}{l} I + V^\top (I - k' U U^\top) V)^{-1} V^\top (I - k' U U^\top) \\
    &= I - k' U U^\top - (V - k' U W) (\frac{1}{l} I + I - k' W^\top W)^{-1} (V - k' U W)^\top \\ 
    &= I - k' U U^\top - l' (V - k' U W) (I - l' k' W^\top W)^{-1} (V - k' U W)^\top.
  \end{align*}
  Unfortunately $W^\top W$ can not be further simplified. The best we can do is to write out a Taylor expansion:
  \[
  (I - l' k' W^\top W)^{-1} = 
  I + l' k' W^\top W + (l' k')^2 (W^\top W)^2 + \ldots.
  \]
  Additionally, $l' k' W^\top W$ is typically not small and so we need lots of terms for this series to be useful.
\end{proof}


==> extended.tex <==
\section{Extended results}
\label{sec:extended}

In this section, we present extended results.

System-level correlation versus instance correlation on summarization.

Table of graphs for other metrics.


==> models.tex <==
\section{\label{sec:models} Evaluation models}
\pl{use term 'surrogate'}
In the previous section, we have observed that the data efficiency of using a model in evaluation is fundamentally limited by the model's correlation with ground truth, as well as annotator variance.
We found that, in theory, with a perfect model, it should be possible halve or even reduce annotation costs by a third.
In this section, we look at a few different evaluation models and report their performance in practice.

Note that while we should still expect evaluation modeling to be difficult, we should hope that it is easier than learning the task itself as we have access not only to the generated utterance but also to existing references that have been rated.

\paragraph{Word-overlap based metrics}
As baseline models we consider using standard automatic metrics such as BLEU, ROUGE, etc.

\paragraph{Sentence embedding models}
Inspired by ADEM, we consider using sentence embedding models and learn the following linear relation between ratings on references:
$g(x,y) \propto \sum_{y_r} f(y_r) * y^\top M y_r$

\paragraph{Task-specific model for MSMarco}
The MSMarco task has the most opportunity for improvements, so we augment a good architecture for the task.

\paragraph{Pretraining}
For each task, we have too little data to learn an entire model, embeddings, so we focus on using the data to fine-tune the model to improve it's correlation. 
To learn the embeddings, we use pretrained models.

Note that we are able to use the labeled data to train our models as long as we use its prediction only on future data. 

\paragraph{Learning optimal scaling using ordinal regression}
Learn how to weigh above features to match ordinal / real-valued ratings.

